Finding Meaningful Distributions of ML Black-boxes under Forensic Investigation

Given a poorly documented neural network model, we take the perspective of a forensic investigator who wants to find out the model's data domain (e.g. whether on face images or traffic signs). Although existing methods such as membership inference and model inversion can be used to uncover some information about an unknown model, they still require knowledge of the data domain to start with. In this paper, we propose solving this problem by leveraging on comprehensive corpus such as ImageNet to select a meaningful distribution that is close to the original training distribution and leads to high performance in follow-up investigations. The corpus comprises two components, a large dataset of samples and meta information such as hierarchical structure and textual information on the samples. Our goal is to select a set of samples from the corpus for the given model. The core of our method is an objective function that considers two criteria on the selected samples: the model functional properties (derived from the dataset), and semantics (derived from the metadata). We also give an algorithm to efficiently search the large space of all possible subsets w.r.t. the objective function. Experimentation results show that the proposed method is effective. For example, cloning a given model (originally trained with CIFAR-10) by using Caltech 101 can achieve 45.5% accuracy. By using datasets selected by our method, the accuracy is improved to 72.0%.

==> future.tex <==
\section{Discussion}
In this section, we discuss potential future work and implications suggested by our work on mitigating adversarial attacks. 
\\ \\
{\em Attack Tracing.\ \ }
    The owner $o$ controls the model distributive process and could distribute distinct model copies to different users $u_i$'s. By controlling over this process, not only does the owner address the challenging issue of preventing adversarial attacks of the models, but the owner could also potentially trace the origin of adversarial samples.

    In our attractor-based solution, the method adds artifacts to influence the model, leading the search process to some local minima or some designated regions. In this process, different attractors are injected into different copies of the model, and each copy will result in different local properties. Thus, it is analogous to a distinct model signature of the various copies. Following this line of thought, it implies that any adversarial sample generated from a particular copy would inadvertently carry a unique imprint of the model's unique properties. Suppose the owner keeps a record of the signatures of the multiple distributed copies. In that case, it could potentially analyze the adversarial sample and ultimately trace it back to the specific model that produced that sample. It would be interesting to investigate further the practicality and efficacy of this adversarial sample tracing.
\\ \\
{\em Attack Deterrence.\ \ } 
    As a consequence of the owner's ability to trace the attack origin, we believe it adds another layer of deterrence to the attack of distributed ML model copies. Firstly, for an adversary who is aware of the traceability of adversarial samples, it causes anonymity issues for the adversary during the distribution of models. The adversary would have to conceal its identity in such a manner that it does not trace back to any related model. Next, since we assume that the users only have black-box access to the distributed models, the variation in each model also increases the cost of the attack. An adversary would have to acquire a large number of different models to replicate the attack among the models, significantly increasing the cost of the adversarial attacks, causing an adversary to think twice about attacking the models distributed models.  


